Improving Automated Code Reviews: Learning from Experience

Modern code review is a critical quality assurance process that is widely adopted in both industry and open source software environments. This process can help newcomers learn from the feedback of experienced reviewers; however, it often brings a large workload and stress to reviewers. To alleviate this burden, the field of automated code reviews aims to automate the process, teaching large language models to provide reviews on submitted code, just as a human would. A recent approach pre-trained and fine-tuned the code intelligent language model on a large-scale code review corpus. However, such techniques did not fully utilise quality reviews amongst the training data. Indeed, reviewers with a higher level of experience or familiarity with the code will likely provide deeper insights than the others. In this study, we set out to investigate whether higher-quality reviews can be generated from automated code review models that are trained based on an experience-aware oversampling technique. Through our quantitative and qualitative evaluation, we find that experience-aware oversampling can increase the correctness, level of information, and meaningfulness of reviews generated by the current state-of-the-art model without introducing new data. The results suggest that a vast amount of high-quality reviews are underutilised with current training strategies. This work sheds light on resource-efficient ways to boost automated code review models.

==> discussion_old.tex <==
\section{Discussion}

\textit{\textbf{RQ1}}. 
Although the upsampling approaches seem to have decreased BLEU-4 \cite{bleu} scores, they have increased in semantic correctness compared to the original approach.
We find this to be true across all partitions of experienced reviewer types, with the largest performance increases being demonstrated in the Major Reviewer demographic.
These findings indicate a potential for better alignment with experienced reviewers' perspectives with our technique.


\textit{\textbf{RQ2}}. 
The amount of information provided within a review comment is not only crucial for guiding the author in performing code refinement correctly, but also vital for knowledge sharing.
The upsampled models have significant increases in suggestion type comments, demonstrating improved inclinations towards providing solutions for developers, whilst at the same time showing less confusion, an anti-pattern that can arise due to lack of experience \cite{antipattern}.
The upsampled models tend to provide explanations more frequently than the original approach, which is especially crucial for aiding the developer's understanding of the issue.


\textit{\textbf{RQ3}}. 
Considering the most critical types of functional issues, more logical, validation and resource related comments could be drawn from the upsampled approaches.
Being rare yet primary concerns of code reviews \cite{microsoftbugs}, the ability to elicit these types of comments show that current automated code review models have the potential to provide more meaningful reviews, that are not just focused on trivial nit pick type issues.
As the underlying dataset is fundamentally unchanged, we demonstrate the existence of vital untapped knowledge within the experienced reviewer partitions of the training data.
As minor reviewer minor authors are the overwhelming majority of the training set, it is crucial to ensure that experienced reviewers' perspectives are not underrepresented.
